Suppression of the Spectral Cross Talk of Optogenetic Switching by Stimulated Depletion Quenching. Theoretical Analysis

Optogenetics is a rapidly growing field of biotechnology, potentially allowing a deeper understanding and control of complex biological networks. The major challenge is the multiplexed control of several optogenetic components in the presence of significant spectral cross talk. We propose and demonstrate through simulations a new control approach of Stimulated Depletion Quenching. This approach is applied to the phytochrome Cph8 bidirectional optogenetic switch, and the results show significant improvement of its dynamic range.

==> ch-OG/App_BG.tex <==
\appendix
\section{Background: The Cph8 Optogenetic Switch}\label{Sec:OG:BGCph8}
Cph8 is a recently developed phytochrome based optogenetic switch designed to control gene expression in E. Coli bacteria \cite{Levskaya2005}. Naturally occurring phytochromes are light sensing proteins in plants, algae, cyanobacteria, and other micro-organisms that harness light as an energy source \cite{Neff2000, Vierstra2000}. These organisms rely on phytochromes to respond to daily and seasonal changes to the light environment. In plants phytochromes control seed development and growth \cite{Franklin2010, Chen2011}, while in algae and cyanobacteria they act as primitive vision sensors to steer toward or away from light during phototaxis \cite{PHP:PHP1481,Garcia2000}. Phytochromes use the photo-isomerization of a covalently attached open-chain tetrapyrrole (bilin) chromophore to reversibly convert between two states in response to light. The chromophore cycles between a dark-stable, red-absorbing $P_R$ state and a meta-stable, far-red-absorbing $P_{FR}$ state, functioning as a molecular switch to regulate numerous responses to light intensity, color, duration, and direction \cite{Smith1995}.

Structurally, phytochromes all share a conserved, modular architecture consisting of an N-terminal photo-sensory module and a C-terminal signal-output module, shown in Figure~\ref{Fig:OG:PhytArch}. The photo-sensory module is made up of three domains: PAS (Per/ARNT/Sim), GAF (cGMP phosphodiesterase/adenylate cyclase/FhlA), and PHY (phytochrome-specific) \cite{Psakis2011}. The bilin chromophore is covalently anchored to a conserved cysteine residue in the GAF domain; and the PAS and GAF domains surround the chromophore, forming the protective binding pocket that isolates the molecule from the surrounding environment, enabling coherent optical interactions within the ``hot, wet, and noisy conditions inside a living cell''\cite{Lloyd2011}. The PHY domain detects the isomerization of the chromophore and mediates the translation of the nanometer scale isomerization of the chromophore into the large scale re-orientation of the remaining phytochrome that can be registered by the cellular signaling architecture and affect biological functions.
\begin{figure}[htb]
	\centering
	\includegraphics[width=.7\linewidth]{ch-OG/Figs/Intro/Fig_PhytArchS}
	\caption[Phytochrome Architecture]{The Cph1 protein complex, divided into the conserved architecture of the canonical phytochrome, which makes up the Photo-Sensory Module of Cph8. The PAS and GAF domains anchor and form the binding pocket around the chromophore phycocyanobilin (PCB). The PHY domain detects the state of the chromophore and passes the information to the Signal Output Module on the other side of the cell membrane, which transforms the information into a cellular signal pathway initiating biological function. (Adapted from \cite{Essen2008})}
	\label{Fig:OG:PhytArch}
\end{figure}
The phytochrome photo-sensory module has a simple modular architecture that shows up naturally in a wide range of species and can be artificially implemented in a number of cell types: including mammalian and bacterial cells \cite{Auldridge2011}. Phytochrome based optogenetic controls seem to be possible in any organism containing the appropriate chromophore (either natively generated, as in many plant and mammalian cells, or exogenously created in bacteria and other cell types) \cite{Burgie2014Rev}. This adaptability and natural wide utility across many cell types will be important for the expansion of phytochrome based switches and the possible multiplexed optical control of multiple switches, which will be expanded upon in Section~\ref{Sec:OG:Conclusions}.

Cph8 is an artificial fusion protein that combines a phytochrome light-sensing domain with a Two Component Signaling system (TCS) native to E. coli.
The phytochrome light sensor is Cph1, originally from the cyanobacterium \emph{Synechocystis PCC6803}, which utilizes phycocyanobilin (PCB) as a chromophore \cite{Gambetta2001}.
The E. Coli TCS is EnvZ, whose normal function is sensing changes in the osmolarity of the surrounding environment \cite{vanAlphen1977}. Under red light illumination the light-sensing domain is excited from the dark stable $P_R$ state to the $P_{FR}$ state, sending a stimulus to the downstream signal output module of the EnvZ half of the Cph8 switch. When activated by stimuli from the sensor domain, EnvZ selectively phosphorylates the OmpR response regulator, a small mobile enzyme in the cell cytoplasm that promotes gene transcription when phosphorylated \cite{Gao2008}. When the switch returns to the $P_R$ state, either by far-red light illuminated or by slow, automatic dark reversion, the EnvZ output module de-phosphorylates the P-OmpR response regulator, inhibiting transcription. The specific gene sequence that OmpR associates with can be engineered into the system. For example, cells have been programmed to generate pigments \cite{Tabor2011} or fluorescent proteins \cite{Schmidl2014} in response to optical switching under exposure to light, so as to provide measurable evidence of the switching function.  A schematic of this TCS system is shown in Figure~\ref{Fig:OG:Cph8Tabor}(a), along with a representative measurement of the light activated production of GFP protein in Cph8 expressing bacteria (b). In Figure~\ref{Fig:OG:Cph8Tabor}(b) the non-zero signal under 650 nm illumination shows the effect of spectral cross-talk (i.e., the system is incapable of being turned off under normal illumination).

\begin{figure}
	\centering
	\includegraphics[width=.7\linewidth]{ch-OG/Figs/Intro/Fig_Cph8Tabor}
	\caption[Cph8 Switching Function]{(adapted from Ref~\cite{Schmidl2014})(a) Schematic of the Cph8-OmpR light-switchable Two Component Sensing system. The sample is exposed to Far-red (740 nm) and red (650 nm) LEDs to initiate switching. Red light partially switches Cph8 from the $P_R$ to $P_{FR}$ form. Far-red light or extended periods of dark conditions revert Cph8 $P_{FR}$ to $P_R$. (b) Mean sfGFP fluorescence of populations of E. coli carrying Cph8-OmpR and illuminated with saturated red and far-red light. Due to spectral cross-talk the GFP signal cannot be fully turned off.}\label{Fig:OG:Cph8Tabor}
\end{figure}

Figure~\ref{Fig:OG:Cph8Spec} (an expansion of Figure~\ref{OG:FullExpConcept}(b))shows the absorption spectra of the Cph8 sample after exposure to red and far-red light until saturation of the photoswitching transition. After far-red exposure the switch has fully converted to the $P_R$ state, as this state does not appreciably absorb at wavelengths longer than 720 nm and there is no forward ($P_R\rightarrow P_{FR}$) photoswitching reaction.
\begin{figure}
	\centering
	\includegraphics{ch-OG/Figs/Intro/Fig_Cph8Spec}
	\caption[Cph8 Absorption]{Absorption spectra of the Cph8 sample.
		The red line shows the spectrum of the pure \pr state, obtained by maintaining the sample under saturated far-red illumination ($\lambda=725$ nm). The purple line is associated with a sample in the photoequilibrium mixed state of 65\% \pr and 35\% \pfr, obtained by maintaining the sample under saturated red illumination ($\lambda=650$ nm). From the difference of these spectra we can extract the pure \pfr spectrum, shown by the dashed blue line. The ultimate goal of this work is clean switching to this projected pure $P_{FR}$ state.}
	\label{Fig:OG:Cph8Spec}
\end{figure}
However, due to overlap of the $P_R$ and $P_{FR}$ absorption spectra at shorter wavelengths, the red light exposure activates both the forward and reverse ($P_{FR}\rightarrow P_R$) photoswitching reactions, and the sample does not fully convert to the $P_{FR}$ state. This photoequilibrium is defined by the ratio of the forward and reverse reaction rates at the excitation wavelength. At 650 nm this equilibrium is 65\% $P_{FR}$, 35\% $P_R$ \cite{Lamparter2002}. This photoequilibrium greatly limits the functional application of these switches (as with the majority of optically sensitive biological molecules) due to the broad overlapping absorption spectra of naturally evolved chromophores.
Stated another way, this spectral cross-talk limits the dynamic range of the switch: the ratio of the final cellular functional output under activating and de-activating light inputs is restricted by preventing the switch from being fully converted to the $P_{FR}$ state.



The source of the spectral cross-talk is the overlap in the absorption spectra of the two chromophore states in the light-sensing module. To increase the dynamic range of the switch we must uncouple the optical interaction with the \pr state (which activates the forward photoswitching reaction) from the optical interaction with the \pfr state (which activates the reverse reaction). We have demonstrated theoretically \cite{ Li2002, Turinici2004, Li2005} and experimentally \cite{ Roth2009, Petersen2010, Rondi2011, Roslund2011, Rondi2012} that even molecules with spectra that are nearly functionally identical can be differentially excited by exploiting their unique, coherent excited state dynamics using ultrashort tailored pulsed light sources. To independently optically address the two states of the Cph8 protein complex we must investigate the photo-isomerization dynamics of the PCB chromophore molecule.


\section{Background: Chromophore Dynamics}\label{Sec:OG:BGPCBDyn}

The chromophore in the photo-sensory module of Cph8, phycocyanobilin (PCB), is made up of four pyrrole rings labeled A-D in Figure~\ref{Fig:OG:PhyPCB}(b) (an expansion of Figure~\ref{OG:FullExpConcept}(a)) in an open configuration joined by conjugated methine bridges. The A-ring of the chromophore is covalently bound to the GAF domain at the Cys259 residue \cite{Essen2008,Lamparter2001}(as shown in Figure~\ref{Fig:OG:PhyPCB}(a)). This domain surrounds the chromophore, forming the binding pocket, which constrains the structure of the chromophore and influences its spectral response and dynamics, while isolating it from environmental disturbances that would destroy the effectiveness of the photo-isomerization reaction. The structure of the chromophore and the surrounding binding pocket shown in Figure~\ref{Fig:OG:PhyPCB}(a) is based on x-ray crystallographic analysis of the Cph1 phytochrome in the \pr state \cite{Essen2008}. The D-ring of the chromophore is less constrained than the rest of the molecule, giving it the freedom of movement to flip between two conformational states.
The planar $ZZZ_{ssa}$ isomer conformation corresponds to the red-light absorbing $P_R$ state. A rotation of the D-ring about the  $C_{15}$=$C_{16}$ carbon bridge flips it out of the plane of the other three pyrroles converting the chromophore to the $ZZE_{ssa}$ conformation associated with the far-red-light absorbing \pfr state. Here $Z(usammen) \& E(ntgegen)$ and $s(yn) \& a(nti)$ refer to the symmetry of the double and single bonds, respectively, of the \emph{C5}, \emph{C10}, and \emph{C15} carbons in the methine bridges joining the four pyrrole rings of the bilin chromophore.
In the $P_{FR}$ state, interaction with the Tyr176 residue of the GAF domain (also labeled in Figure~\ref{Fig:OG:PhyPCB}(a)) affects down stream changes in the rest of the phytochrome, converting the nanometer scale isomerization of the chromophore into a large-scale re-distribution of neighboring domains producing a signaling pathway that can influence cellular function.
The optical characteristics of the chromophore are very sensitive to the binding pocket: mutation of alleles in the PAS and GAF domains of the phytochrome can prevent photoswitching or shift the absorption spectrum by up to 30 nm \cite{Shcherbakova2016}. In spite of these shifts, the change in the central wavelength is always smaller than the broad, overlapping absorption spectrum characteristic of the bilin chromophores, meaning it is still susceptible to spectral cross-talk. However, it should be noted that while not sufficient to distinguish species by linear absorption, these subtle shifts to the chromophore binding pocket should provide an ultimate basis to exploit pulse shaping for optimal dynamic discrimination (ODD) of multiple similar switches (see Section~\ref{Sec:OG:Conclusions}).

\begin{figure}
	\centering
	\includegraphics[width=.8\linewidth]{ch-OG/Figs/Intro/Fig_PhyPCB}
	\caption[Chromophore Structure and Isomerization]{(a) (Adapted from \cite{Essen2008}) Ribbon representation structure of the binding pocket in the GAF domain of the Cph1 photo-sensory module. The PCB chromophore is covalently attached to the GAF domain at C-259. The tyrosine residue Y176 is believed to help stabilize the $P_{FR}$ state and is important in the photoswitching reaction. (b) PCB Chromophore in the $P_R$ and $P_{FR}$ states. The $C_{14}\!\!-\!\!C_{15}$=$C_{16}$ methine bridge linking the C-ring and D-ring is highlighted. The two states partially interconvert with red light (650 nm), and concomitantly under far-red light (720 nm) or dark-reversion. }\label{Fig:OG:PhyPCB}
\end{figure}

As discussed above, the absorption of the $P_{FR}$ state extends to longer wavelengths than $P_R$, yielding near complete ($>$97\%) conversion from the $P_{FR}$ to the $P_R$ state (the reverse reaction) under constant far-red excitation. The opposite reaction is challenging due to spectral cross-talk: the red light excitation is absorbed by both the $P_R$ and $P_{FR}$ states.
Since we cannot solve the problem of spectral cross-talk by altering the absorption spectra, we must turn to an alternate set of optical interactions to find suitable controls to differentiate the states. While the ground state absorption of the $P_R$ and $P_{FR}$ states are similar and overlapping, the excited state dynamics are very different and open a new avenue for controlling the chromophores and differentiating the two states. Thus, we seek to exploit the distinct dynamics of the forward and reverse photo-isomerization reaction to halt the reverse reaction while minimizing the impact on the forward reaction.

The photo-isomerization of the PCB chromophore in both directions is initiated by photo-excitation of the molecule, immediately followed by very rapid coherent vibronic relaxation on the excited state surface \cite{Heyne2002}. This sequence is then followed by a portion of the excited molecules transitioning to a transient intermediate product state beginning the isomerization. The remaining excited state population returns to its respective initial ground state. In the forward isomerization reaction ($P_R\rightarrow P_{FR}$) this intermediate is LUMI-R; in the reverse ($P_{FR}\rightarrow P_R$) the intermediate is LUMI-F \cite{Bischoff2000,Bischoff2001}. These two transient intermediate species are unique to the forward and reverse reaction, respectively, and the subsequent relaxations progress along distinct, separate reaction coordinates.  The LUMI-R and LUMI-F transient intermediate products persist for several nanoseconds and trigger a series of large scale conformational reorganizations of the protein residues in the downstream domains to complete the photoswitching transformation between the $P_R$ and $P_{FR}$ states of the full Cph8 switch. The names ``\pr'' and ``\pfr'' are used to refer to the red-light and far-red-light absorbing states, respectively, of the PCB chromophore, the phytochrome light-sensing module, and the overall Cph8 switch depending on context.

The initial coherent steps of the ultrafast photo-isomerization are not as well understood as the slower domain reorganizations associated with the latter steps of the switching. It is generally agreed that the isomerization in both directions is initiated when the PCB chromophore absorbs a photon of light, exciting an electron from the $\pi$-conjugated system primarily localized on the C and D pyrrole rings and the methine bridge that joins them. This promotes an electron to the anti-bonding $\pi$* orbital, weakening the double bonding character of the $C_{15}$-$C_{16}$ carbon atoms in the bridge (labeled on the chromophores in Figure~\ref{Fig:OG:PhyPCB}(b)), enabling rotation of the outer D ring and inter-conversion between the $P_R$ state and the $P_{FR}$ state, and vice versa, by way of non-shared transient intermediates. \cite{Bischoff1998, Bischoff2001, Heyne2002}. It is here that the forward ($P_R\rightarrow P_{FR}$) and reverse ($P_{FR}\rightarrow P_R$) photo-isomerization reactions start to differ and also where the disagreements about the earliest dynamics of the excited state relaxation begin.
In particular, the early stage dynamics of the initial excited state relaxation and isomerization steps of the Cph1 phytochrome have been studied using numerous ultrafast electronic \cite{Heyne2002, Fitzpatrick2012, Kim2012} and vibrational \cite{Dasgupta2009, vanWilderen2009, vanThor2007, Yang2012} transient spectroscopies, often arriving at different and sometimes even contradictory conclusions.
In all reported studies, analysis of time-resolved spectra reveal complex multi-exponential excited-state relaxation dynamics, but there are different interpretations of these measurements. The extent of the isomerization reaction occurring on the excited state and the homogeneity of the ground state population are the principle areas of disagreement.
There are two schools of thought with regard to ground state population:
(1) there is an ensemble of ground state sub-populations that each undergo distinct single-exponential dynamics after excitation (the “inhomogeneous perspective”), and
(2) there is a single uniform ground state population and the complex, non-exponential excited state dynamics are due to multiple vibronic resonances at a conical intersection (the “homogeneous perspective”).

Each perspective is supported by a number of experimental studies using a variety of measurement techniques. Resonant Raman intensity analysis \cite{Spillane2009} and hybrid quantum mechanics/molecular mechanics (QM/MM) simulations \cite{Mroginski2010}support a homogeneous \pr state that undergoes multi-phasic excited state dynamics. Solid-state NMR resolved two distinct ground state \pr sub-populations: one structure consistent with the known crystal structure and a second interpreted as having a modified charge distribution and hydrogen bond network \cite{Song2011}. Some pump-dump-probe (PDP) studies find evidence of a homogeneous ground state in $P_R$ \cite{vanWilderen2009, Fitzpatrick2012}, while other PDP experiments observe a heterogeneous ground state in Cph1 \cite{Kim20140618,Kim2013,Kim2012}and in a related phytochrome \cite{Chang2013}. There is currently no consensus as to the exact nature of the ultrafast dynamics of the photo-isomerization.
The results of the most recently published experiments characterizing the forward and reverse photo-isomerization reactions are summarized below.

The forward photo-isomerization of $P_R$ to $P_{FR}$ of the Cph1 phytochrome has been characterized by the Larsen group from UC Davis \cite{Kim20140417}. The study consists of a combination of temperature-dependent and excitation-wavelength-dependent static and ultrafast transient absorption measurements. Using a global analysis of the combined measurements they resolve five distinct ground state sub-populations (Pr1, ..., Pr5) co-existing at thermal equilibrium, each undergoing single-exponential dynamics through separate excited and intermediate states. The sub-populations can be grouped into two distinct categories: the fast-decaying photo-active populations (Pr1 and Pr5) and the slow-decaying fluorescent populations (Pr3-Pr5). The exponential lifetimes associated with each sub-population at room temperature are summarized in Figure~\ref{Fig:OG:Larsen}. The time scale of the forward isomerization is given by the formation of LUMI-R in 61 picoseconds.


\begin{figure}
	\centering
	\includegraphics[width=5in]{ch-OG/Figs/Intro/Fig_Larsen}
	\caption[Forward photoswitching dynamics reveal Heterogeneous $P_R$ Ground State]{(adapted from~\cite{Kim20140417}) Measurements of forward photoswitching dynamics reveal heterogeneous ground state sub-populations. The photoswitching population (${P_r2}$ above) forms the LUMI-R intermediate isomerization product with a time constant of 61 ps.}\label{Fig:OG:Larsen}
\end{figure}

The reverse ($P_{FR}\rightarrow P_R$) photo-reaction has been less thoroughly studied due to the transient nature of the $P_{FR}$ state and inability to fully remove the confounding $P_R$ state. In a collaboration between the Heyne group at the Freie Universitat Berlin and the Mathies group at UC Berkeley, a combination of Femtosecond Stimulated Raman Spectroscopy (FSRS) and polarization-resolved transient IR spectroscopy was used to map the initial steps of the reverse photo-isomerization reaction from the $P_{FR}$ state of the Cph1 phytochrome \cite{Yang2016}. Researchers detected the extremely rapid sub-picosecond development of the LUMI-F intermediate product. This observation is supported by direct measurement of the orientation of the chromophore D-ring by the femtosecond resolved polarization anisotropy of the $C_{19}$=O vibrational absorption (a good indicator of the orientation of the ring) as shown in Figure~\ref{Fig:OG:HeyneMathies}(a-c). The FSRS measurement of the $C_{15}$=$C_{16}$ stretch in Figure~\ref{Fig:OG:HeyneMathies}(d) shows the shift to lower wavenumber of the stretching vibration, which reflects a reduction in the vibrational force constant after relaxation from the FC region. The inset of Figure~\ref{Fig:OG:HeyneMathies}(d) shows the ground-state recovery dynamics of the 1607 $cm^{-1}$ bleach feature fit to a bi-exponential decay curve with time constants of $t_1$=(300$\pm$50) fs and $t_2$=(6$\pm$3) ps, representing a $\approx$70\% loss of the excited population within a picosecond of excitation; in agreement with the timescale of the ring flip given by the IR measurement.


\begin{figure}
	\centering
	\includegraphics[width=.95\linewidth]{ch-OG/Figs/Intro/Fig_HeyneMathies}
	\caption[Reverse photoswitching reaction involves complex excited state dynamics]{(adapted from~\cite{Yang2016}) (a-b) Measurements and analysis of the polarization resolved transient IR absorption and (d) FSRS measurements of the reverse photo-isomerization of PCB in Cph1 phytochrome. (a) Ultrafast transient absorption of the ground state $\nu (C_{19}$=$O)$ and $\nu (C_{19}$=$O)$* vibrational modes on the electronic ground and excited state energy surfaces. Black dots in (a) represent IR probe polarization parallel to the visible excitation, while red circles represent perpendicular probe polarization. The vertical blue bars illustrate that the difference between the two polarized absorption signals remains fixed in the ground state, but rapidly changes in the excited state. This provides direct measurement of the rotation of the ($C_{19}$=O)* vibrational mode and, by extension, the D-ring of the chromophore.
		(b) The polarization anisotropy quantifies the difference between the two polarized absorption signals and is a measure of the angle between the transition dipole moments of the electronic excitation and the vibrational mode. The time varying anisotropy of the excited state ($C_{19}$=O)* mode is strong evidence of rotation of the D-ring in the excited state with a time constant of 0.7 ps.
		(c) Charts of the shift in peak FSRS frequency of the excited state $C_{15}$=$C_{16}$ stretch associated with a weakening of the bond order after excitation. The inset shows the ground-state bleach dynamics for the $C_{15}$=$C_{16}$ stretch, exhibiting bi-exponential recovery of the ground state over two time domains: a fast 300 fs recovery and a slower 6 ps recovery. These figures are a condensed selection of many measurements from reference~\cite{Yang2016} which support the conclusion of sub-picosecond coherent isomerization in the reverse ($P_{FR}\rightarrow P_R$) photoswitching reaction.}\label{Fig:OG:HeyneMathies}
\end{figure}

Analysis of multiple vibrational modes on the chromophore and the direct measure of the ultrafast change in the polarization anisotropy of the $C_{19}$=O on the D-ring support sub-picosecond isomerization of the PCB chromophore to the LUMI-F transient photo-product. The ultrafast structural change in the bilin chromophore may indicate formation of the first intermediate state on the excited state potential surface, and is accelerated by a non-bonding “methyl-methyl clash” of the outer methyl groups on the C-ring and D-ring in the $P_{FR}$ ground state. A representation of the excited state dynamics on a 2-D potential energy surface is shown in Figure~\ref{Fig:OG:HMConInt}. The relaxation from the initial Frank-Condon excitation point ($P_{fr}^*$  in Figure~\ref{Fig:OG:HMConInt}) occurs in 300 fs, at which point the molecule either relaxes back to the $P_{FR}$ ground state or remains on the excited surface, depending on whether its D-ring has initiated rotation. Those chromophores remaining in the excited state continue to rotate until reaching the conical intersection with the LUMI-F photo-product surface over the next 700 fs. The conical intersection mediates the rapid generation of the LUMI-F photo-product.
\begin{figure}
	\centering
	\includegraphics[width=.8\linewidth]{ch-OG/Figs/Intro/Fig_HeyneMathiesConInt}
	\caption{(adapted from~\cite{Yang2016}) (a) Sketch of the multi-dimensional potential energy surface representative of the isomerization reaction, which is shown on the right (b). Non-bonding interactions between the methyl groups on the C and D rings (indicated with green ``\textcolor[rgb]{0,0.6,0}{\textbf{)(}}'' in (b)) place a strain on the \pfr ground state which enhances the speed of the reverse isomerization once initiated by absorption of a photon. The important vibrations that are part of the reaction coordinate in the multi-dimensional PES are depicted on the axes in (a). The two-step mechanism of the isomerization process is depicted by the black and red trajectories. The conical intersection, denoted by a grey square, enables very fast generation of the LUMI-F photoproduct and $P_{FR}$ ground state.}\label{Fig:OG:HMConInt}
\end{figure}


These studies inform our understanding of the Cph8 switch and guide the development of the experiment reported in this chapter. While the exact details of the excited state dynamics are neither fully understood nor agreed upon, this situation does not hinder our ability to conduct experiments exploring a pathway to the control of the optogenetic switches.
The ability to distinguish the two states of the Cph8 switch does not require exact knowledge of the coherent excited state dynamics of the molecule, only the ability to interact with the system while the excited state coherent dynamics are ongoing.
Built on the essence of the background experiments reported here, a kinetic-based model may be constructed using the generalized switching picture captured in Figure~\ref{OG:FullExpConcept}(c) (Section~\ref{Sec:OG:REMSim}). We will see that, there are inherent features of the photo-physics in the latter figure (i.e., the stability of the two switch states, and the irreversibility of the switching dynamics once initiated) that are amenable to identifying the per-exposure iterative map for the transfer of population between the switch states.
The existence of this iterative map is more important than a detailed quantitatively accurate model.
The experiments in this work (Section~\ref{Sec:OG:SDQExp}) will identify the map from the laboratory data, and then use the properties of the iterative map to calculate the effective transfer for the $P_R \rightarrow P_{FR}$ photoswitching reaction.
Importantly, the conclusions drawn from these initial experiments should apply to further advanced studies, including pulse-shaping assisted multiplexed optimal dynamic discrimination of multiple similar optogenetic switches.





==> ch-OG/Sec_Intro-Sims.tex <==
%\singlespacing

\section{Introduction and Background}\label{Sec:OG:IntroBG}


\subsection{Introduction}\label{Sec:OG:Introduction}

%\doublespacing

The variety and complexity of tasks performed by living cells is astonishing: they harvest and refine chemicals from their environment \cite{Albertsch2}, synthesize complex chemicals in response to demand \cite{Gething1992}, respond to changes in their environments in ways that mirror logic and memory \cite{HOPFIELD199453}, self-replicate and multiply under globally limited constraints \cite{AlbertsEssentials,Ardissone2016}, and work together - communicating and combining to form multi-cellular tissues \cite{Albertsch19}.
A cell accomplishes all these tasks by measuring an array of internal and external environmental conditions using various sensor protein complexes and performing a specific biological function in response, as dictated by a set of instructions in its genetic code. In this way, cells behave as functional machines, performing actions in direct response to stimuli.
Recently, biologists have developed the capability to genetically engineer cells, supplanting the natural sensors with light sensitive proteins. These engineered proteins enable the activation or suppression of specific cellular functions with optical signals, turning a piece of the naturally developed sensing-response system into an externally accessible ``control panel''.
This breakthrough, called \emph{optogenetics} \cite{Deisseroth2011, Pastrana2011}, enables the precise and reversible control of specific biological processes in living cells by external optical stimuli to systematically perturb the system and observe its response\cite{Fenno2011}.

Currently available optogenetic tools can control a range of biological processes including ion channel activation
%(enabling its primary application as a high fidelity neuromodulation technique
(enabling high fidelity neuromodulation \cite{Zemelman2002, Boyden2005, XiangLi2005}), organism mobilization \cite{Wen2012, Leifer2011, LeiferPhD2011} and behavior \cite{Montgomery2015, Gunaydin20141535, Husson2013},
protein synthesis in cells \cite{Olson2012,Tabor2011},
%
% Optogenetic control is typically mediated by
gene expression or inhibition \cite{Shimizu-Sato2002, Konermann2013, Cao2013, Tyszkiewicz2008},
protein localization at specific cell sites \cite{Levskaya2009, Toettcher20131422, Toettcher2011, Toettcher2011409, Leung02092008},
or sequestration of active proteins away from their site of reaction \cite{Lee2014, Yang01082013}.
Optical techniques can be very appealing for the control and monitoring of biological systems, with many advantages over physical or chemical/pharmacological activation.
Light is a noninvasive tool that interacts strongly with specific biologically relevant molecules and can be applied with high spatial and temporal resolution.
Precise activation signals can be encoded into many controllable parameters of the optical signal, including the light's intensity, frequency spectrum, phase structure, and the duration or temporal pattern of the exposure. Moreover, optical stimuli can be rapidly halted, in contrast to diffusionally controlled chemicals.

In spite of these favorable aspects, the practical implementation of optogenetics is prevented from reaching its fullest potential by spectral cross-talk: the overlapping optical responses of the switches.
Most chromophores, the molecules within the optogenetic switch that absorb light, have broad, featureless absorption spectra, which limits the number of switches that can be independently addressed by linear photo-excitation.
More problematic is that for many switches even the absorption spectrum of the activated and de-activated states overlap, preventing the switch from being completely converted from one state to the other.
This inability to distinguish the two states of the switch limits the accessible dynamic range of the system and fidelity of control.

The capability now exists to overcome the spectral cross-talk: it has been shown that even molecules with nearly identical static absorption spectra can exhibit unique dynamical responses to ultrashort laser pulses \cite{Courvoisier2006}.
These distinguishable dynamics can be accentuated by a set of optimal optical control pulses to distinguish similar molecular species, this technique is known as Optimal Dynamic Discrimination (ODD) \cite{Li2002, Turinici2004, Li2005,Roth2009, Petersen2010, Rondi2011, Roslund2011, Rondi2012,Goun2016}.
By interacting with the time-dependent non-linear optical response of a molecule, rather than just the static absorption spectrum, we increase the number of control parameters that can be varied to search for orthogonal optical controls that are not restricted by the same spectral cross-talk as the linear optical responses.
In principle, a suitable set of orthogonal optical controls should be capable of separating the optical responses of several similar optogenetic switches that would be extremely difficult to independently address by conventional linear photo-excitation.
The ultimate goal of this research is the simultaneous (multiplexed) control of multiple optogenetic switches over their maximum dynamic range, thereby independently and simultaneously controlling a large number of cellular functions.
In the present work we take the first step toward the goal of multiplexed control of multiple optogenetic switches by developing a model to simulate the optical interaction between such pulses and a simplified optogenetic switch. Results with this model indicate that the dynamic range of the switch can be enhanced beyond the linear photoequilibrium limit imposed by spectral cross-talk.


The simplified optogenetic switch modeled in this paper is based on Cph8, a phytochrome based red/far-red sensing optogenetic switch developed for controlling gene expression in E. Coli bacteria \cite{Levskaya2005, Tabor2009,Tabor2011}.
More detailed information about the Cph8 switch and the dynamics of its internal chromophore \emph{phycocyanobilin} (PCB) will be provided in Appendices \ref{Sec:OG:BGCph8} and \ref{Sec:OG:BGPCBDyn}. 
%To summarize briefly:
Cph8 is an artificial ``fusion'' protein, a synthesis of the light sensing domains of the Cph1 protein originally found in Cyanobacteria with the Histidine-Kinase Two-Component Switch (TCS) signalling domains of EnvZ, a protein native to E. Coli that is associated with gene transcription \cite{Schmidl2014}.
The chromophore in the Cph8 switch, phycocyanobilin (PCB), converts between two states by photo-isomerization, as shown in Figure~\ref{OG:FullExpConcept}(a).
The gene-expressing ``On'' state absorbs red light and is called \pr, while the biologically inactive ``Off'' state is called \pfr because its absorption spectrum is shifted to longer wavelengths in the far-red. The absorption spectra of these two states is shown in Figure~\ref{OG:FullExpConcept}(b).
\begin{figure}
  \centering
  \includegraphics[width=5.9in]{ch-OG/Figs/Intro/ExpConcept_2}
  \caption[Overview of Experimental Concept]{
  	Overview of the Controlled Optogenetics experimental concept: (a) Photoswitching of Cph8 is initiated by photo-isomerization of the PCB chromophore between an active state $(P_{R})$ and an in-active state $(P_{FR})$. The \pfr state can be completely removed with far-red light, however spectral cross-talk prevents complete removal of the \pr state. 
  	(b) Absorption spectra of a sample of Cph8 in the pure 100\% \pr state, the photoequilibrium mixed state of 65\% $P_{FR}$/35\% $P_{R}$, and the pure 100\% \pfr state that we aim to reach by Stimulated Depletion Quenching (SDQ) enhancement.
  	(c)\emph{SDQ Concept:} The Cph8 sample in a mix of \pr and \pfr states is exposed to ultrashort Excitation and Depletion pulses, separated by a delay $\uptau$. Both states are excited and undergo dissimilar coherent ultrafast excited state dynamics along a chromophore isomerization coordinate to either the transient product states (LUMI-R and LUMI-F) or back to their initial ground states (grey arrows). The transient products more slowly transform the remaining protein domains downstream of the chromophore, completing the photoswitching reaction.
  	Precision timing of the depletion pulse permits the selective transfer of a larger portion of the $P_{FR}$* molecules back to the $P_{FR}$ ground state (i.e., quenched molecules no longer follow grey dashed arrows) compared to the same process for $P_R$*, thereby quenching the reverse reaction more than the forward. This process shifts the equilibrium of the photoswitching reaction toward \pfr, increasing the dynamic range of the Cph8 switch.
}
  \label{OG:FullExpConcept}
\end{figure}
The Cph8 switch can be fully converted from the \pfr state to the \pr state by continuous illumination with far-red light ($\lambda \geq$ 720 nm), this is described as the ``reverse'' photo-isomerization reaction.
Deactivation of the switch, converting from the \pr state to the \pfr state, is described as the ``forward'' photo-isomerization reaction, and due to the overlapping absorption spectra of the two states there is no wavelength of light that will initiate the forward photo-isomerization reaction without also initiating the reverse reaction.
The simultaneous photo-reaction between the two states under red-illumination comes to photoequilibrium with a maximum \pfr population of $\sim65\%$ (\pr$\sim35\%$). The absorption spectrum of a sample in this equilibrium mixed state is also shown in Figure~\ref{OG:FullExpConcept}(b).
%\tcb{The goal of this research is to push past this linear photoequilibrium threshold and achieve nearer to 100\% \pfr.}
Using ultrashort laser light pulses we will exploit the unique dynamic optical responses of the \pr and \pfr states to selectively ``quench'' the reverse photoswitching reaction, $P_{FR} \rightarrow P_R$, by stimulated depletion, shifting the photoequilibrium to increase the dynamic range of the switch.




A schematic of the proposed \emph{Stimulated Depletion Quenching (SDQ)} mechanism is shown in Figure~\ref{OG:FullExpConcept}(c), and will be more fully explained in Section~\ref{Sec:OG:ExpDesc}.
To summarize, the actuation of the Cph8 switch is initiated when the PCB chromophore absorbs a red or far-red photon.
%and an electron is excited from the highest conjugated $\pi$-orbital of the molecule to an anti-bonding $\pi$*-orbital. This process weakens the bond order of the methine bridge joining the outer C and D rings of the chromophore, resulting in molecular isomerization by rotation of the D-ring, producing an irreversible cascade of down-stream protein domain reorganizations converting that single electronic excitation into the activation of a cellular signaling pathway.
This excitation weakens the bond order of the methine bridge joining the outer C and D rings of PCB, resulting in molecular isomerization by rotation of the D-ring, producing an irreversible cascade of down-stream protein domain reorganizations converting that single electronic excitation into the actuation of a cellular signaling pathway.
Due to spectral cross-talk of the \pr and \pfr states both are excited by photons of red light, it is not possible to prevent these unwanted electronic excitations of the \pfr state of the PCB chromophore.
% with conventional direct radiative absorption.
% and the switch can never be fully turned off by conventional light exposure. an equilibrium concentration of activated switches always persists.
%One potential means of eliminating spectral cross-talk would entail re-engineering the photo-sensory domain to alter the absorption spectrum of the chromophores. Accomplishing this without diminishing the effectiveness of the signaling pathway is challenging, and has not been accomplished at the current time. Furthermore, even if the states of an individual switch could be distinguished, any attempts to utilize multiple optogenetic switches or to use them in concert with fluorescent reporters would quickly run into the same problem of spectral cross-talk due to the inherent limited fidelity and range of the single parameter of excitation/emission wavelength.
However, it \emph{is} possible to prevent the switching of the remainder of the Cph8 protein complex and subsequent activation of the cellular signaling pathways by de-exciting the chromophore before the larger protein ``notices'' that it has been triggered.
After the excitation to the $P_{R}^\ast$ or $P_{FR}^\ast$ state there is a brief interval of time before the chromophore begins isomerization. During this interval the molecule can be returned to its initial state by stimulated depletion, making it appear as though no absorption had occurred and quenching the photoswitching reaction.
%To maintain the optical control of the system in this approach, the excited electron would be transferred to the ground state by stimulated emission.
Further, to facilitate this capability, there should be sufficient differences in the excited state dynamics and stimulated emission spectra of the two forms of the chromophore to preferentially depopulate the $P_{FR}$* excited state over that of the $P_R$* excited state, allowing the forward reaction to proceed while quenching the reverse reaction.
This selective quenching shifts the photoequilibrium of the simultaneous forward and reverse photoswitching reactions, thereby increasing the maximum attainable $P_{FR}$ population.
The total photoswitching reaction can be represented by a simple linear transformation map for an incremental $P_R \rightarrow P_{FR}$ step per laser interaction; upon repeated iteration of the mapping transform (i.e., repeated laser exposure) the full transition of large populations of the Cph8 switch from the \pr to the \pfr state can be accomplished. The components of the transformation map can be calculated from a small number of measurements of the system, enabling us to rapidly calculate the photoequilibrium population and the enhancement of the dynamic range accessible by the Cph8 switch brought on by the SDQ mechanism.

The experimental research described here is a feasibility study of this proposed SDQ mechanism, aiming to demonstrate control of the photo-isomerization reaction in the Cph8 optogenetic switch by achieving greater stimulated depletion quenching of the reverse photoswitching reaction compared to the forward reaction by harnessing the unique dynamics of the two photo-isomerization pathways.
This work has a limited goal, but represents an important first step toward the ultimate goals of achieving maximal dynamic range control of a single optogenetic switch and simultaneous independent control of multiple optogenetic switches in living cells by multiplexed, optimal non-linear photoswitching.


%The chapter is organized as follows.
The remainder of this introduction section contains additional background information on the Cph8 phytochrome based switch (Section~\ref{Sec:OG:BGCph8}), the photo-isomerization of the PCB chromophore associated with Cph8 (Section~\ref{Sec:OG:BGPCBDyn}), and a more detailed description of the proposed SDQ technique (Section~\ref{Sec:OG:ExpDesc}).
Section~\ref{Sec:OG:REMSim} describes a model for simulations assessing the feasibility of the experiment and exploring the significant reduced parameter space to determine an effective range of experimental parameters.
Section~\ref{Sec:OG:SDQExp} presents the experimental controlled photoswitching of the Cph8 system and the procedure for data processing and analysis of the resulting measurements.
These processed data are further analyzed and results are presented in Section~\ref{Sec:OG:Results}, followed by a discussion of the current results and recommended future experimental directions in Section~\ref{Sec:OG:Conclusions}.


%Photoswitching from the ``ON state'' to the ``OFF state'' (the so-called ``forward reaction'') is often achieved by the same wavelengths of light as the ``reverse reaction" (``OFF'' to ``ON'') due to the overlapping absorption spectra of the states.

%\section{Background}\label{Sec:OG:BG}
\subsection{Description of the SDQ Mechanism}\label{Sec:OG:ExpDesc}

%\begin{figure}
%  \centering
%  \includegraphics[width=.65\linewidth]{ch-OG/Figs/ExpConcept_Schem}
%  \caption[Diagram of Experimental Concept]{Diagram of SDQ Experimental Concept: The Cph8 sample is exposed to the ultrashort Excitation and Depletion pulses, separated by $\uptau_{Delay}$. Both initial states of the switch are excited and the molecules undergo ultrafast relaxation toward the branching conical intersection to either the transient product states (LUMI-R and LUMI-F) or back to the initial ground states. There is good spectral overlap of the depletion pulse with the $P_{FR}$* excited state depletion spectrum (red arrow connects surfaces) and poor overlap with the $P_{R}$* depletion spectrum (red arrow too short to connect surfaces). A barrier on the $P_R$* excited surface slows the forward reaction. The combination of spectral overlap and timing permit the depletion pulse to coherently and selectively drive a larger portion of the $P_{FR}$* excited molecules back to $P_{FR}$ ground state, quenching the reverse reaction more than the forward. (the quenched molecule no longer follows the path of the grey dashed arrows)}\label{Fig:OG:ExpConcept}
%\end{figure}

In this experiment selective stimulated emission is employed to coherently transfer PCB chromophores initially excited to the $P_{FR}$* state back to the \pfr ground state before isomerization can occur, while simultaneously allowing chromophores initially excited to the $P_{R}$* state to persist and undergo photoswitching to the $P_{FR}$ state.
The concept of this SDQ mechanism is represented in the diagram in Figure~\ref{OG:FullExpConcept}(c).
The sample is exposed to two ultrashort laser pulses: an excitation pulse and a depletion pulse.
The spectrum of the excitation pulse overlaps with the absorption spectra of both the $P_{R}$ and $P_{FR}$ states of the PCB chromophore. Exciting the molecule with the ultrashort pulse creates corresponding coherent wave packets from superpositions of vibrational levels on the electronic excited state surfaces of both forms of the chromophore.
These wave packets undergo dissimilar coherent dynamics as they relax from their initial Frank-Condon excitation states toward a coherent vibronic transition through a conical intersection either back to their initial ground state or to a transient intermediate photo-product state.
Before the molecules complete these dynamics, a second pulse arrives after a short, controlled delay ($\uptau_{Delay}$).
This depletion pulse has a central wavelength set to overlap more favorably with the stimulated emission spectrum of the $P_{FR}$* state than the $P_{R}$* state.
The combination of spectral overlap and timing permit the depletion pulse to selectively drive a larger portion of the $P_{FR}$* excited molecules back to the $P_{FR}$ ground state, preferentially slowing the reverse photo-isomerization reaction while allowing the forward reaction to continue transferring some portion of the \pr population to the \pfr state.
Those molecules remaining in either of the excited states after the depletion pulse continue their unperturbed dynamics, either isomerizing to the transient photo-product state or returning to their initial ground state.
%The relative final populations of the Cph8 switch in each state after being exposed to the pulsed excitation and depletion sequence are measured by absorption spectroscopy.

SDQ shares many similarities with Stimulated Emission Depletion (STED), a common super-resolution imaging technique used in microscopy. In STED microscopy the suppression of fluorescence from a ring-shaped outer spot provides contrast to an un-depleted inner spot, yielding an instrument response function with sub-diffraction limited spatial resolution.
%When using STED on specialized dyes, complete suppression of the fluorescence signal is possible.
In both STED and SDQ the goal is to fully de-populate an excited electronic state before the system can relax by an undesired pathway. However, there is a critical difference between conventional STED of a fluorescent molecule and our proposed SDQ of the excited state of a photoswitch.
% that may prevent us from achieving the same degree of complete de-population of the excited state.The non-radiative photo-isomerization of the chromophore in the Cph8 sensor domain module is very different from emission of a dye or fluorescent protein. In fact, there is a class of Phytochrome-based fluorescent proteins designed specifically by disabling the photoswitching and blocking the isomerization of the chromophore in the sensor domain module, forcing the excited chromophore to decay back to the ground state by spontaneous emission \cite{Zhu2015, Shcherbakova2015, Shcherbakova2016 }.
%
In most fluorescent species the lifetime of the excited electronic state exceeds the lifetime of the coherent vibrational states by several orders of magnitude. In these species the molecule vibrationally relaxes to a stationary state on the electronic excited surface and a (relatively) long depletion pulse can interact with the population over an extended period, maximizing the population transferred to the ground state.
%
As discussed in Section~\ref{Sec:OG:BGPCBDyn},the vibrational and electronic excited state lifetimes are of similar duration for the chromophores,
and it is believed the molecule undergoes semi-coherent vibronic dynamics throughout the isomerization/relaxation (i.e., the initially coherent superposition persists while also interacting with the surrounding protein and solvent environments in ways which support the coherence or induce decoherence, the details of which are presently not well characterized \cite{Spillane2012,Mroginski2010}).
%from the instant the wave packet is formed on the excited state surface until it either returns to its initial ground state or transitions to the intermediate state that proceeds to isomerization and protein switching.
This impacts the potential effectiveness of the proposed SDQ mechanism in two ways.
First, because the excited state lifetime is so much shorter than a fluorescent species, the depletion pulse interacts with the molecule for less time, likely reducing the maximum achievable depletion.
Second, because the population is never in a stationary state on the excited surface, the depletion pulse must interact with a spectrally shifting wave packet, possibly negatively impacting the coherent transfer to the ground state.
Future experiments should be able to overcome both of these obstacles by utilizing pulse shaping and feedback control to discover suitable pulse shapes for the excitation and depletion pulses that accommodate or exploit the excited state dynamics of the $P_{R}$* and $P_{FR}$* states in a maximally distinguishable fashion.
To demonstrate that even without optimally tailored pulse shaping the extremely rapid dynamics of the photo-isomerization would not prevent the SDQ mechanism from controlling the optogenetic switching of Cph8, in Section~\ref{Sec:OG:REMSim} we run simulations with a model system exhibiting comparable optical response and dynamics upon exposure to the dual-pulse excitation-depletion sequences employed in the experiments of Section~\ref{Sec:OG:SDQExp}.

In practical applications, optogenetic switches are expressed in large numbers in genetically targeted cells \cite{Mohanty2015}, not as isolated molecules. Optogenetic control of cellular processes involves the global photoswitching of a large population of protein switches from an arbitrary initial distribution of states to a maximally active or inactive population, restricted by the Maximal Dynamic Range (MDR) of the system and light exposure condition.  This will necessarily be a gradual transfer of population between states over many laser exposure iterations.
In particular, the low quantum efficiency of the photoswitching reaction (10-20\% in both reaction directions \cite{Yang2016}), as well as the fact that not all of the molecules will absorb photons in a single exposure, means that it would not be possible to transfer the entire population of a group of switches to a desired final state in one pulsed laser iteration.
The iterative transfer of population is made possible by the relative stability of both active and inactive states in phytochrome-based switches, allowing the state distribution to persist between laser exposure iterations. The \pfr state of Cph8 is meta-stable, reverting to the \pr state in the dark, but at such a slow rate (variable in different implementations and environments, from many seconds to many hours \cite{Olson2014}) that the state distribution can be said to be constant between laser pulses repeated at more than a few Hertz.
Each laser exposure iteration transfers a fraction of the proteins from one state to the other, with a per exposure fractional yield that is independent of the states' populations, defined exclusively by the characteristics of the light.
Because of the stability of the product state of the photoswitching reactions, we are able to transfer large populations of switches to the desired product state in many small steps.
This iterative transfer of population is important for a mechanism like SDQ, which acts by inhibiting an undesired reaction pathway rather than enhancing the rate of a desired pathway. The SDQ mechanism, while reducing the per-exposure fractional yield of the photoswitching reaction will none the less positively impact the final photoequilibrium after many exposures, which is the feature of interest for the practical implementation of controlled photoswitching.


In this work, the excitation and depletion pulse parameters will be varied to determine the wavelengths, powers, pulse durations, and delay timings which selectively deplete the $P_{FR}$* level most effectively, quenching the reverse reaction while minimally hindering the forward reaction.
This exploration of the experimental control parameter space aims to be a feasibility study for the proposed mechanism, identifying a path through the vast, unexplored control landscape toward a region amenable to effective control of the photoswitching reaction, thereby laying the foundation for more sophisticated optimal control experiments on optogenetic switches in the future.




==> ch-OG/Sec_Results.tex <==
%\singlespacing

\subsection{Results and Analysis}\label{Sec:OG:Results}




%% Done with section ====================================================================================== 

==> ch-OG/Sec_SDQExp.tex <==
%\singlespacing

\section{Experimental Control of photoswitching by Stimulated Depletion Quenching (SDQ)}\label{Sec:OG:SDQExp}

%\doublespacing
The simulations presented in Section~\ref{Sec:OG:REMSim} predict that the SDQ mechanism effectively halts the reverse photoswitching reaction of the Cph8 optogenetic switch while allowing the forward photoswitching reaction to continue, shifting the photoequilibrium and increasing the maximal dynamic range accessible by the switch after many laser exposure iterations.
In this section we experimentally utilize the SDQ technique to enhance the control of the Cph8 photoswitching reaction.
These experiments determine the Optical Transformation Matrix (OTM) iterative map associated with a particular laser control parameter set by measuring a group of \emph{characteristic coefficients}, the analog of the same process in the simulations, to calculate the final photoequilibrium populations after many of exposures to the associated laser control pulses.
Further, we characterize the dependence of the SDQ enhancement on the experimentally variable laser control parameters, comparing the measured dependence to the results of the simulated parameter space survey of Section~\ref{Sec:OG:REMSurvey} and determining the most effective exposure conditions for maximizing the dynamic range of the switch.
%The parameters varied in the simulated survey of Section~\ref{Sec:OG:REMSurvey} were chosen to reflect the experimental parameters examined in the following experiment.
The results of these experiments, presented in Section~\ref{Sec:OG:Results}, are in qualitative agreement with the results of the rate equation model (REM) simulations of the last section, and confirm the feasibility of the optimal control of the photoswitching reaction in Cph8 by the SDQ mechanism, laying the ground work for further experiments incorporating pulse shaping and closed-loop optimization to achieve higher fidelity control of optogenetic switches.
%%
%%




%\singlespacing

\subsection{Experimental Apparatus} \label{Sec:OG:Apparatus}

%\doublespacing

A diagram of the laser sources and optics for the generation, conditioning, and routing of the excitation and depletion pulses to the Sample Flow Circuit (SFC), where the Cph8 sample is stored and circulated for exposure and measurement, are presented in Figure~\ref{Fig:OG:ApparatusLasers}. A more detailed diagram of the SFC is shown later in Figure~\ref{Fig:OG:ApparatusFluidCircuit}. The primary laser source for this experiment is a Ti:Sapphire regenerative amplifier (Coherent Legend) generating high intensity, ultrashort-pulse 800 nm laser pulses of duration $\sim$35 fs (50 nm spectral bandwidth) with average pulse energy 2.1 mJ/pulse and 1KHz repetition rate. This source beam is split evenly by a high damage threshold, low GVD 50:50 beam splitter to generate the excitation and depletion beams.
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{ch-OG/Figs/Exp/Fig_AppLasers}
  \caption[Experimental Schematic]{Schematic of experimental setup including light sources for excitation and depletion laser pulses, beam routing and pulse conditioning optics, sample flow circuit (dotted box, see detailed diagram in Figure~\ref{Fig:OG:ApparatusFluidCircuit}), and systems for aligning, synchronizing, characterizing, and observing beams.}\label{Fig:OG:ApparatusLasers}
\end{figure}

The excitation beam is generated in a Topaz-White Non-collinear Optical Parametric Amplifier, which is configured to generate pulses with energy of $\sim$20 $\mu$J/pulse and spectral range from 550-780 nm, peaking at 580 nm. The NOPA beam is filtered with a 610 nm long-pass glass absorption filter and a 650nm short-pass interference filter angle tuned to give a maximum wavelength of 640 nm, producing a nearly constant intensity spectrum from 610 nm to 640 nm. This filtered beam is temporally compressed at the sample exposure site (after passing through all routing optics) by maximizing SHG bandwidth and intensity in a thin 100 $\mu$m thick $\beta$-BBO crystal. The pulse is compressed by adjusting an internal Bi-Prism compressor in the TOPAS–White NOPA.

The depletion beam is generated by spectrally filtering a portion of the Ti:Sapphire amplifier beam using short-pass and long-pass interference filters.
The depletion quenching was analyzed at two wavelengths: 835 nm, corresponding to the peak depletion wavelength predicted by the REM simulations in Section~\ref{Sec:OG:REMSurvey}, and 775 nm, corresponding to the shortest useable wavelength of the Ti:Sapphire amplifier.
We compare the measured depletion quenching at these two wavelengths to the REM simulations.
The longer wavelength depletion beam was generated using a 860 nm 40 nm wide band-pass interference filter angle-tuned to pick out the red edge of the Ti:Sapphire amplifier spectrum, producing a pulse with spectral width of 10 nm centered at 835 nm. The shorter wavelength depletion beam was similarly generated with with a 780 nm, 10 nm wide band-pass interference filter angle-tuned to be centered at 775 nm.
%directly when within its spectral range or by directing a fraction of the amplifier to a Palitra  Optical Parametric Amplifier (OPA) which generates pulses with energy of over 200 $\mu$J/pulse and in a signal beam that can be tuned over a spectral range from 1.0 $\mu$m to 3 $\mu$m, this signal beam can be mixed with the 800 nm Ti:Sapph beam by Difference Frequency Mixing followed by Second Harmonic Generation in BBO to produce a depletion beam that can be scanned from 850 nm to 3 $\mu$m}. The spectrum of the depletion beam is defined and cleaned up with a series of bandpass, shortpass, and longpass interference filters
The filtered depletion beam was then sent through a dual prism stretcher to adjust the pulse length. The depletion pulse is stretched to enhance the stimulated depletion transition efficiency.

The TOPAS-White NOPA is designed to maximize the possible bandwidth of the output and thereby produce the shortest pulsed output.
To accomplish this, the device incorporates a grating-based pulse shaper on the supercontinuum seed beam that conditions the seed for amplification, uses cylindrical optics throughout to maximize beam energies without burning the nonlinear crystal, and employs ``tilted-pulse beam mixing" \cite{Riedle2000} in the amplification crystal. Tilted-pulse  beam mixing compensates a degree of angular dispersion across the beams that are accumulated when the beams enter the mixing crystal and allows greater phase matching bandwidth (similar to the way in which a non-collinear OPA has greater phase matching bandwidth than a collinear OPA). These options increase the spectral range, minimum pulse width, and total power of the NOPA pulse; but, they do so at the expense of the spatial mode of the beam, which can be decidedly distorted at the output, as indicated in Figure~\ref{Fig:OG:SpatialFilter}. Because the non-linear optical effects exploited in the following experiments are very sensitive to the intensity distribution and beam quality we apply a spatial filter with a 100 $\mu$m pinhole. This cleans up the NOPA beam to a smooth Gaussian spot at the expense of laser power. The throughput of the spatial filter is typically $\sim$35\%.

\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{ch-OG/Figs/Exp/Fig_OG_SpatialFilter}
  \caption[Effect of Excitation Beam Spatial Filter]{Effect of the spatial filter: (a) Image of the NOPA output, showing the beam distortion characteristic of device construction. (b) Image of Airy disk formed with pinhole spatial filter. The central spot is used for the experiment and outer rings are blocked by an iris. The smooth beam profile is critical for reliable measurements.}
  \label{Fig:OG:SpatialFilter}
\end{figure}

To ensure that the depletion spot size at the sample is much larger than the excitation spot (ensuring that the entire excited sample is uniformly exposed to the depletion pulse) there is an adjustable beam reducing telescope near the beam combiner in the depletion beam line. This telescope can be adjusted while monitoring the overlapped spots at the sample on a camera imaging the exposure spots to confirm proper coverage.

Both beams pass through adjustable delay lines to synchronize the pulses. A computer controlled micrometer driven delay stage is placed in the excitation beam line to introduce a precise delay between the excitation and depletion pulses for time-resolved studies. The computer controlled delay stage can vary the delay over 150 ps in 3 fs steps (25 mm travel in 0.5 $\mu$m steps), though most measurements described in the following sections are made between $\pm$2 picoseconds of excitation/depletion synchronization.

The two beams are independently attenuated with neutral density filters to set the exposure intensity before being spatially combined on an 800 nm long-pass interference filter at 45$\deg$ to transmit the depletion beam and reflect the excitation beam, using close positioned steering mirrors to accurately align the overlap and direction of each beam.
After the beams are combined they can be focused into the microchannel exposure cell, or to check their alignment and synchronization they can be redirected through alternate beam lines by a series of removable flip-up mirrors.
A spatial overlap beam line sends the beams through multiple irises over a path length of more than 2 meters to ensure their collimation and collinearity in the near and far field.
A temporal overlap beam line sends the beams through a thin $\beta$-BBO crystal (100 $\mu$m thick) for synchronization of the pulses by Sum Frequency Generation (SFG) as well as compression of each beam by maximization of Second Harmonic Generation (SHG) intensity and bandwidth. The $\beta$-BBO crystal must be very thin to maximize phase matching across the (considerable) spectral range of the two pulses. Once synchronized by SFG, the excitation-depletion delay is set by the computer controlled delay stage.

At this stage, once excitation and depletion pulses overlap in time and space, the beams are focused into the exposure cell by an achromatic doublet with focal length 150 mm (the lens and mirrors preceding the exposure cell are replicated in the synchronization beam line to compensate for dispersion effects). The focusing beams are reflected off a small silver coated turning prism mounted at the center of a 2 inch diameter high numerical aperture (NA) lens before the exposure cell. This lens images the microchannel cell and laser spots onto a video imaging system which monitors the sample and can be used for fine alignment of the focal spots. This high NA lens is also used to collect fluorescence from the microchannel cell in measurements of Stimulated Emission Depletion of Fluorescent Proteins used to align and characterize the instrument response function of the apparatus. The combined beams are focused onto the exposure cell and the cell is brought forward so that the excitation beam diameter is approximately 50\% larger than the microchannel flow cell width and the depletion beam diameter is approximately 50\% larger than the excitation spot. Images of the microchannel and focused beams from the video monitor are shown in Figure~\ref{Fig:OG:FocalSpots}. The spot sizes of the beams are set such that all material flowing through the channel width is exposed to the laser excitation and depletion pulses with similar intensity and no portion at the sides of the flow cell is left unexposed.

\begin{figure}
  \centering
  \includegraphics[width=3.5in]{ch-OG/Figs/Exp/Fig_OG_BeamSpots}
  \caption[Focal Spots on Microchannel Exposure Cell]{Images of the microchannel exposure cell with the excitation and depletion beam spots imaged at the channel depth of the cell. The camera is a monochromatic CMOS chip, so the laser spot images were collected separately, then colored and layered on top of each other with photo-editing software to form the composite image above. The black lines through the spots show the edges of the 100 $\mu m$ wide channel. }\label{Fig:OG:FocalSpots}
\end{figure}


A more detailed diagram of the Sample Flow Circuit (SFC) is presented in Figure~\ref{Fig:OG:ApparatusFluidCircuit}. The protein sample circulates in a minimal volume continuously flowing fluid circuit to ensure each measurement is made on a fresh sample and to mitigate sample photo-damage. The SFC is driven by a piezoelectric micro-pump (Takasago fluidics) and consists of a glass reservoir where the bulk of the sample is held, a microchannel exposure cell where the laser activated photoswitching occurs, and a fluid filled optical fiber absorption cell (WPI LWCC-M-50) where the final yield of the photo-reaction (degree of Cph8 switching between $P_{R}$ and $P_{FR}$ states) can be measured, all connected by narrow PTFE tubing  to minimize dead volume.
\begin{figure}
  \centering
  \includegraphics[width=.85\linewidth]{ch-OG/Figs/Exp/Figure_OG_ApparatusFluidCircuit}
  \caption[Detailed View of Apparatus Sample Flow Circuit System]{Diagram of SFC which circulates the solution containing the Cph8 protein. Laser exposure initiating the photo-isomerization reaction takes place in the microchannel exposure cell, a 100 $\mu$m wide microfluidic channel that flows the sample through the laser focus. Measurement of photo-reaction product yield is done in the absorption cell, a fluid filled optical waveguide allowing for long path (5 cm) measurements of low volume (12 $\mu$L) samples. Further description of system provided in the text.} \label{Fig:OG:ApparatusFluidCircuit}
\end{figure}

The reservoir is under continuous far-red illumination by a 'reset diode' emitting 730 nm light (M730D2, Thorlabs) which maintains the Cph8 protein in the sample solution in an initial $P_{R}$ state.
There is a white light source that shines on a transparent section of tubing connecting the micro-pump to the exposure cell. This ‘actinic’ light source can be turned on to pre-switch a portion of the molecules before they reach the exposure cell, initializing the sample in a mixture of the $P_{R}$ and $P_{FR}$ states. This initial $P_{FR}$ population is related to the flow rate (exposure time) and lamp intensity, and can be variably set to give an initial (\pr, \pfr) population up to $\sim (55,45)\%$.
The initial state of the sample is maintained below the linear photoequilibrium of 65\% \pfr because the goal of the experiment is to determine the OTM map, which requires accurate measurement of the per-exposure yield and quenching coefficients. Near photoequilibrium the per-exposure yield is very small, and difficult to accurately measure.
%The upper limit is due to the combination of short exposure time and broad lamp spectrum; filtering the spectrum decreases back reaction from \pfr at the expense of lamp intensity producing approximately the same maximum \pfr.

The exposure cell is a 100 $\mu$m wide 300 $\mu$m deep microchannel flow cell (Translume Inc.). This narrow channel concentrates the sample into the small area of the laser focal spot, ensuring that the excitation beam completely covers the channel cross-section while still being focused tightly enough to drive the necessary optical transitions.
This exposes the entire flowing volume to a consistent exposure dose set by the laser intensity and fluid flow rate.
This experimental configuration also has similarities to ‘lab-on-chip’ bio-circuits used in synthetic biology,which is a field making practical application of optogenetic switching to manipulate and harness cellular function.

The long path absorption cell is a micro-fluidic waveguide capillary cell (LWCC-M-50, WPI inc) that allows highly precise measurements of absorption spectra in low volumes of sample by using the analyzed liquid sample as the internal media in a liquid core optical fiber, keeping the light in contact with the sample by total internal reflection at the liquid-core interface and enabling long optical path lengths. The total internal volume of the absorption cell is 12 $\mu$L.
The sample is probed with a stabilized Tungsten white light lamp (Thorlabs SLS202) that provides a smooth, continuous spectrum well-suited to absorption measurements. The light source is stabilized by an electronic feedback circuit to provide $<$0.1\% optical power drift per hour for long term stability. The light source is coupled to the LWCC by a fiber optic cable, and the transmitted probe is coupled to a compact spectrometer (Ocean Optics MAYA4000) by another fiber optic cable. This system gives a simple, accurate, and rapid measurement of the sample absorption spectrum.

%\singlespacing

\subsection{Data Collection and Initial Processing}\label{Sec:OG:DataProc}

%\doublespacing

Using the apparatus described in the last section, the sample is (i) circulated as absorption spectra (like those shown in Figure~\ref{Fig:OG:AbsSpec}) are continuously measured, (ii) analyzed to extract the absolute concentration of the two conformational states of Cph8, (iii) saved by the computer, and (iv) indexed by their time of acquisition. As the laser exposure conditions are varied, the collected absorption spectra and relative photoswitching reaction product populations change in response, as shown later in Figure~\ref{R1}.
Despite not having knowledge of the time dependent excited-state level populations, as we did in the simulations of Section~\ref{Sec:OG:REMSingle}, we are still able to extract useful information about the ultrafast interactions between the molecular switch and the excitation and depletion pulses. By varying the experimental laser control parameters and measuring the final photoswitching reaction product states under a series of six \emph{Exposure Conditions} (described in Table~\ref{Tab:OG:ExpCond}) from the final product state populations we may calculate a set of six \emph{characteristic coefficients} (described in Table~\ref{Tab:CharCoeff}). Just as in the simulations of Section ~\ref{Sec:OG:REMSingle} these \emph{characteristic coefficients} are a series of reaction coefficients that quantify the effects of the excitation and depletion pulses in ways that facilitate analysis and allow us to build the OTM map to calculate the enhanced photoequilibrium populations.

\begin{figure}
  \centering
  \includegraphics[width=.9\linewidth]{ch-OG/Figs/Data/AbsSpec}
  \caption[Representative Absorption Spectra from Cph8]{(a) Representative absorption spectra of Cph8 taken in the absorption cell under typical experimental concentrations and conditions. This graph contains spectra from Cph8 in a `pure' \pr state and a mixed state of 71.5\% $P_{R}$ and 28.5\% $P_{FR}$. (b) The mixed state spectrum is fit to a linear combination of the reference spectra and a nonlinear background (BG). Dashed traces show the relative contribution of the \pr and \pfr states to the total absorption fit curve (black trace). }\label{Fig:OG:AbsSpec}
\end{figure}

Representative absorption measurements from two samples are shown in Figure~\ref{Fig:OG:AbsSpec}(a), while Figure~\ref{Fig:OG:AbsSpec}(b) shows the fitting of one of these absorption measurements to known reference spectra to extract the concentrations of the component states present in the sample.
The two samples shown in Figure~\ref{Fig:OG:AbsSpec}(a) include a sample in the pure \pr state (red trace) under continuous illumination at 730 nm as well as a sample with a mixed population containing Cph8 in both \pr and \pfr states (orange trace) produced by white light illumination.
Reset samples in the `pure' \pr state typically retain a small residual population of $1-3\%$ \pfr.
Backgrounds have been subtracted to place these two spectra on the same baseline.

The measured absorption spectra are fit to a linear combination of absorption peaks and a third order polynomial background:
%\tcg{(Equation~\ref{Eq:OG:FitFun} below)to extract the absolute concentrations of the individual components that making up the sample}:
\begin{equation}\label{Eq:OG:FitFun}
  S(\lambda, c_i)=c_{R}S_{R}(\lambda)+c_{FR}S_{FR}(\lambda)+c_{R'}S_{R'}(\lambda)+c_{W}S_{W}(\lambda)+\sum_{n=0}^{3}c_n\cdot(\lambda-\lambda_0)^n
\end{equation}
\noindent The four absorption peaks are the known reference spectra of Cph8 in the \pr and \pfr states ($S_{R}(\lambda)$ and $S_{FR}(\lambda)$) (measured independently and verified by comparison to ref~\cite{Lamparter2001}), a small water overtone peak at 970 nm ($S_{W}(\lambda)$), and a  blue-shifted sub-population of $P_{R}$-Cph8 with a spectrum peaking at 655 nm that develops over the course of experiments ($S_{R'}(\lambda)$). This sub-population is discussed further below.
This analytical function is fit to the data by an unconstrained least squared residual fitting algorithm.
The reference spectra in Equation~\ref{Eq:OG:FitFun} are scaled to the known extinction coefficients found in the literature \cite{Lamparter2001} and multiplied by the optical path length of the absorption cell (5 cm), so the fit coefficients $c_R$, $c_{R'}$, and $c_{FR}$ correspond to absolute concentrations of the component states of Cph8 in Molar units.
The analytical fit to the spectrum of the mixed state sample is shown in Figure~\ref{Fig:OG:AbsSpec}(b), the fit curve (thin black trace) is in good agreement with the measured absorption data (thicker orange trace). The spectra of the individual components of the mixture are also shown in the figure, superimposed on the calculated background curve (dashed curves). The calculated total Cph8 concentration is 2.21 $\mu M$, and the white light illumination has converted 28.5\% of the sample to the \pfr state, leaving 71.5\% in the \pr state.

When excited by the ultrashort laser pulses, the dynamics of the chromophore molecule -- and subsequently the photoswitching reaction product distribution of the sample -- are intimately coupled to the complex spectral phase and temporal field shape of the excitation and depletion pulses interacting with the system.
The high-dimensional parameter space that characterizes these pulses is immense (especially when unconstrained shaping of the spectral/temporal phase of the pulses is employed to tailor the pulsed laser field profile, which is not employed at this stage of experimentation).
In this initial feasibility study we limit our exploration of this vast control space to perform a reduced survey of the key control parameters that are expected to be most relevant to the photo-isomerization dynamics of the PCB molecule and the Cph8 system, parallelling the survey of simulated results performed in Section~\ref{Sec:OG:REMSurvey}.
%The laser control parameters chosen to experimentally survey are the same onces explored in the simulated parameter space survey, and the experimental results presented .......
This procedure lays the ground work for future experiments using optimally tailored pulse shaping to exploit the coherent ultrafast excited state dynamics of the switches.

The set of experimentally controlled parameters investigated include: the average power of the excitation and depletion beams ($\langle P_{Ex}\rangle$ and $\langle P_{Dp}\rangle$), the central wavelength and bandwidth of the excitation pulse spectrum (($\lambda_0^{Ex}$,$\Delta\lambda_{Ex}$) and depletion pulse spectrum ($\lambda_0^{Dp},\Delta\lambda_{Dp}$)), the laser pulses' temporal widths ($\Delta t_{Ex}$ and $\Delta t_{Dp}$)
%~\footnote{(as described in Section~\ref{Sec:OG:Apparatus} pulse widths are set by an internal bi-prism pair inside the NOPA for the excitation pulse and the dual prism stretcher shown in Figure~\ref{Fig:OG:ApparatusLasers} for the depletion pulse, though there are plans to use coherent pulse shaping in future experiments to generate more elaborate complex tailored pulse shapes)},
the time delay between the two pulses ($\uptau_{(Ex,Dp)}$), and the sample flow rate (q), which (in conjunction with the laser repetition rate) defines the number of laser pulses the sample is exposed to as it passes through the laser focal spot in the microchannel exposure cell.
Apart from the flow rate, these parameters are the same set used to define the simulated excitation and depletion pulses in Section~\ref{Sec:OG:REMSingle}.
This set of experimental control parameters,
\begin{align}\label{exExpContParam}
    \left[\langle P_{Ex}\rangle, \lambda_0^{Ex}, \Delta\lambda_{Ex}, \Delta t_{Ex}, \langle P_{Dp}\rangle, \lambda_0^{Dp},\Delta\lambda_{Dp}, \Delta t_{Dp}, \uptau_{(Ex,Dp)}, q\right],
\end{align}
\noindent defines a single point in the high-dimensional parameter space to manipulate the molecular switch.
The molecular response is related to all of these parameters collectively through coupled, complex relationships.
In this experiment we begin to survey a portion of this parameter space, guided by the results of the rate equation model simulations of Section~\ref{Sec:OG:REMSim}, which provided an initial starting point for these experimental measurements.
%By surveying this predicted region of enhancement we confirm the experimental feasibility of the SDQ mechanism and begin to compile a map of this parameter space that leads to the control parameter sets which increase the functional dynamic range of the Cph8 optogenetic switch. This lays the foundation for future experiments to utilize the tools of optimal feedback control by tailored ultrashort pulses to reach the global optimum laser exposure that will fully maximize the optogenetic switch dynamic range.


As in Section~\ref{Sec:OG:REMSingle}, we define the final product populations of the photoswitching reaction as a linear transformation from the initial state population distribution using a set of \emph{characteristic coefficients}:
\begin{subequations}\label{eqSMFCC}
  \begin{align}
    P_{R,f}={}&\left(1-D_R-(1-Q_R ) Y_{R,FR} \right)P_{R,i} + \left((1-Q_{FR} ) Y_{FR,R} \right)P_{FR,i} \\
    P_{FR,f}={}&\left((1-Q_R ) Y_{R,FR} \right)P_{R,i} + \left(1-D_F-(1-Q_{FR} ) Y_{FR,R} \right)P_{FR,i}
\end{align}
\end{subequations}
%\begin{align}\label{eqSMFCC}
%    [P_{R}]_{f}={}&\left(1-D_R-(1-Q_R ) Y_{R,FR} \right)[P_{R}]_{i} + \left((1-Q_F ) Y_{FR,R} \right)[P_{FR}]_{i}\\
%    [P_{FR}]_{f}={}&\left((1-Q_R ) Y_{R,FR} \right)[P_{R}]_{i} + \left(1-D_F-(1-Q_F ) Y_{FR,R} \right)[P_{FR}]_{i}
%\end{align}
The forward and reverse Yield and Quenching coefficients are defined as they were before in Equation~\ref{eq:Sim:CharCoeffs} of Section~\ref{Sec:OG:REMSingle}. The per exposure yield in the forward direction, ${Y_{R,FR}}$, is the fraction of molecules transferred from \pr to \pfr by the excitation pulse alone with no depletion and the forward quenching coefficient, ${Q_R}$, is the relative change in forward yield brought on by the dual pulsed excitation-depletion sequence.
The corresponding coefficients ${Y_{FR,R}}$ and ${Q_{FR}}$ are defined for the reverse reaction in the same way.
There is an additional pair of experimental \emph{characteristic coefficients} not present in the simulations of Section~\ref{Sec:OG:REMSim}, ${D_{R}}$ and ${D_{FR}}$, associated with the loss of protein within the sample due to photo-damage by the high intensity laser pulses. Care was taken to minimize photo-damage by limiting peak laser intensities, but it is a loss channel that must be accounted for in the experimental measurements.
%These six coefficients are functionally dependent on the variable experimental control parameters listed above and characterize the photoswitching reaction, quantifying the features of interest for maximizing the functional dynamic range of the switches.


Because we do not have knowledge of the transient populations of the LUMI-R/LUMI-F intermediate product states as we did in the simulations of Section~\ref{Sec:OG:REMSim} we can not use these values to define the \emph{characteristic coefficients} as we did there.
Rather, to calculate these six unknown coefficients we measure the final product populations under series of six \emph{Exposure Conditions} (described and collected in Table~\ref{Tab:OG:ExpCond}).
The sample can be left to circulate with no laser exposure, measuring the initial population distribution in either the pure-\pr (EC1, $\binom{R_0}{F_0}$) or mixed (EC4, $\binom{R_{M0}}{F_{M0}}$) initial conditions.
From either of these initial conditions the sample can be exposed to the excitation laser alone (EC2, $\binom{R_{Ex}}{F_{Ex}}$;EC5, $\binom{R_{MEx}}{F_{MEx}}$), providing the linear photoswitching reaction products, or the excitation-depletion pair (EC3, $\binom{R_{ED}}{F_{ED}}$;EC6,  $\binom{R_{MED}}{F_{MED}}$), producing the non-linear SDQ-enhanced photoswitching reaction products.
These six \emph{Exposure Conditions} make up a ``\emph{Full Data Set}'', thereby producing sufficient measurements to calculate the full set of \emph{characteristic coefficients} for a specified laser control parameter set.
From the photoswitching reaction products starting in the pure \pr condition we calculate the yield, quenching, and damage coefficients of the forward reaction.
Using the final product states collected starting in the mixed condition and the calculated forward characteristic coefficients we can calculate the reverse yield, quenching, and damage coefficients.
The set of six \emph{characteristic coefficients} is collected in Table~\ref{Tab:CharCoeff} along with their relation to the measured final product populations under the six \emph{Exposure Conditions}.

% TABLE EXPOSURE CONDITIONS
\begin{table}
\centering
\footnotesize
	\begin{tabular}{>{\centering\arraybackslash}p{.30in}| @{}>{\centering\arraybackslash}m{.85in}@{}|@{} >{\centering\arraybackslash}m{.85in} @{}| m{3.6in} }
\toprule
\toprule

\textbf{EC\#} &
\makecell{\textbf{Initial} \\ \textbf{State} $(\mu M)$}&
\makecell{\textbf{Final} \\ \textbf{State} $(\mu M)$}&
\textbf{Description of Exposure Condition} \\

\midrule

1& &$\begin{bmatrix} R_{\text{\tiny 0}} \\ F_{\text{\tiny 0}} \\ \end{bmatrix}$&
\uline{Pure $P_R$ state:} Reservoir under continuous 730 nm diode illumination to hold switch in $P_R$ state. (typically $1-3\%$ \pfr remains).\\
2&\makecell{$\begin{bmatrix} R_{0} \\ F_{0} \\ \end{bmatrix}$ } &$\begin{bmatrix} R_{\text{\tiny Ex}} \\ F_{\text{\tiny Ex}} \\ \end{bmatrix}$&
\rule{0pt}{3ex} \uline{Linear Excitation:} Sample exposed to excitation laser alone. Change in $P_{FR}$ gives forward yield ($Y_{R,FR}$), while difference in $P_{FR}$ produced and $P_R$ lost gives forward damage coefficient ($D_R$).\\
3& &$\begin{bmatrix} R_{\text{\tiny ED}} \\ F_{\text{\tiny ED}} \\ \end{bmatrix}$&
\rule{0pt}{3ex} \uline{Excitation+Depletion:} Sample exposed to Excitation and Depletion pulse pair to excite and then quench forward reaction ($Q_R$). Power, spectrum, and timing of pulses are varied to map dependence of $Q_R$.\\
\midrule
4& &$\begin{bmatrix} R_{\text{\tiny M0}} \\ F_{\text{\tiny M0}} \\ \end{bmatrix}$&
\uline{Mixed Initial State:} Dual pre-illumination (730 nm diode+white lamp) prepares sample in mixed initial state. $[P_{FR}]_{init}$ dependent on lamp intensity and sample flow rate.\\

5&$\begin{bmatrix} R_{\text{\tiny M0}} \\ F_{\text{\tiny M0}} \\ \end{bmatrix}$&$\begin{bmatrix} R_{\text{\tiny MEx}} \\ F_{\text{\tiny MEx}} \\ \end{bmatrix}$&
\rule{0pt}{3ex} \uline{Mixed Linear Excitation:} Sample with initial $P_{FR}$ population undergoes forward and reverse reaction. Using the calculated $Y_{R,FR}$ the reverse yield ($Y_{FR,R}$) can be extracted.\\

6& &$\begin{bmatrix} R_{\text{\tiny MED}} \\ F_{\text{\tiny MED}} \\ \end{bmatrix}$&
\rule{0pt}{3ex} \uline{Mixed Excitation+Depletion:} Sample undergoing forward and reverse reaction is exposed to depletion pulse. Using the calculated $Y_{R,FR}$, $Y_{FR,R}$, \& $Q_R$, the Reverse Quenching Coeff. ($Q_{FR}$) can be extracted.\\	

\bottomrule
	\end{tabular}
	\caption[Exposure Conditions]{Exposure conditions to calculate Characteristic Coefficients from measured final product states. The six exposure conditions defines a \emph{Full Data Series} for a single control parameter set. The Full Data Series is required to calculate the full set of \emph{Characteristic Coefficients} for that set of control parameters; though, useful information about individual characteristic coefficients can be extracted from partial data series.}
	\label{Tab:OG:ExpCond}
\end{table}

% TABLE CHARACTERISTIC COEFFICIENTS
\begin{table}
\centering
\renewcommand{\arraystretch}{1.5}
\footnotesize
\begin{tabular}{>{\centering\arraybackslash}m{1.2in} >{\centering\arraybackslash}m{0.7in} >{\centering\arraybackslash}m{3in} }
\toprule
\toprule

\textbf{Characteristic\break Coefficients}& \textbf{Symbol} & \nohyphens{\textbf{Calculation from Measured\break Final Product Concentrations}}\\
\midrule
Forward\break Yield&$Y_{R,FR}$&${(F_{Ex}-F_0)}/{R_0}$\\
    \hline
Forward\break Damage&$D_R$&$1-Y_{R,FR}-R_{Ex}/R_0$\\
    \hline
Forward\break Quenching&$Q_R$&$1-(\nicefrac{(F_{ED}-F_0)}{R_0} )/Y_{R,FR}$\\
    \hline
Reverse\break Yield&$Y_{FR,R}$&$\dfrac{R_{MEx}-R_{M0} (1-Y_{R,FR}-D_R )}{F_{M0}}$\\
    \hline
Reverse \break Damage&$D_{FR}$&$1-\dfrac{F_{MEx}+R_{MEx}-(1-D_R)R_{M0}}{F_{M0}}$\\
    \hline
Reverse\break Quenching&$Q_{FR}$&$1- \dfrac{R_{MED}-R_{M0}(1-(1-Q_R )Y_{R,FR}-D_R )}{Y_{FR,R}\cdot F_{M0}}$\\
\bottomrule
        %\end{center}
		\end{tabular}
	\caption[Characteristic Coefficients]{The Characteristic Coefficients relate the measured
  final photoswitching reaction products to the ultrafast interactions being used to control the process.
  The first and second columns give the name and symbols for each coefficient, while the last column describes the method of calculating the coefficient from the final product state populations measured under the exposure conditions in Table~\ref{Tab:OG:ExpCond}.}
  \label{Tab:CharCoeff}
%\end{center}
\end{table}

Once these \emph{characteristic coefficients} are calculated, we can form an Optical Transformation Matrix (OTM), just as we did in Equation~\ref{eq:OG:OTMccs} in Section~\ref{Sec:OG:REMMulti}:

%\singlespacing
\begin{equation}\label{eq:OG:expOTMccs}
%\small
 \begin{bmatrix}
          P_{R,f} \\
          P_{FR,f} \\
        \end{bmatrix} =\begin{bmatrix}
                        (1-(1-Q_{R})Y_{R,FR}) & (1-Q_{FR})Y_{FR,R} \\
                        (1-Q_{R})Y_{R,FR} & (1-(1-Q_{FR})Y_{FR,R})
                      \end{bmatrix} \begin{bmatrix}
          P_{R,i} \\
          P_{FR,i} \\
        \end{bmatrix}
\end{equation}

%\doublespacing

\noindent The damage coefficients are omitted from the OTM, as the inclusion of the loss term prevents calculation of the steady-state equilibrium solution from the eigensolutions (as no steady-state exists and the sample continuously loses population). Rather, accounting for the damage coefficients in the calculation of the other \emph{characteristic coefficients} ensures their accuracy.
%, and the decimation count (the time it takes to reach photoequilibrium) is compared to the
With the experimentally measured OTM we can calculate the eigensolutions of the matrix, as we did in Section~\ref{Sec:OG:REMMulti}, to determine the projected photoequilibrium from the eigenvector with eigenvalue $\lambda_{eq}=1$.
Comparing the decimation count, $N_{DEC}$, associated with the second eigenvalue of the OTM to the sample loss associated with the damage coefficient indicates the amount of sample lost to damage in the number of iterations it would take to reach the projected photoequilibrium. %These projected equilibrium product state populations allow us to estimate the effectiveness of a laser excitation-depletion pulse pair outside the limits of our experimental setup.
\emph{It is important to note that the calculation of the steady-state equilibrium population distribution from the OTM is independent of the rate equation model used in Section~\ref{Sec:OG:REMSim}, and not limited by it's approximations.
The use of the transformation matrix is a fundamental consequence of the linear transformation of the sample from an initial distribution to a final distribution by an iterated forward and reverse transfer pathway on a conserved total population.}

A \emph{Full Data Set} is defined by measuring the final product concentrations under all six of the exposure conditions in Table~\ref{Tab:OG:ExpCond} for a given control parameter set (see Figure~\ref{R2}).
Each time one of the control parameters in the set is varied a Full Data Set is measured to extract the \emph{characteristic coefficients} at that point in the parameter space landscape before moving on to the next point in the survey.
%As long as the experimental conditions remain consistent, the measurements of the exposure conditions need not be done sequentially, and typically several values of experimental control parameters are measured in sequence at a particular exposure condition (i.e. while measuring the Excitation+Depletion conditions, a number of pulse delays or powers could be measured before moving to the next condition).
The \emph{characteristic coefficients} build on each other, with each requiring the value of the previous determined coefficient, thus making it critical that experimental conditions remain consistent throughout the measurement of each full data series. In the current construction of the apparatus it is still difficult to maintain constant and fully reproducible experimental conditions, limiting the quantitative precision and reproducibility of calculated results measured at different times and on different samples.
However, the experimental conditions are sufficiently stable to measure several \emph{Full Data Sets} under consistent conditions, and the relationships between the characteristic coefficients calculated from these measurements show clear conserved trends across all the measurements.

%==========================================================================
%==================================================================================
%==================================================================================
\subsection{Representative Data Series}

In Figure~\ref{R1} we present data collected from a portion of a typical measurement series, taken over the course of one hour.
The absolute concentration of the states of Cph8 in the sample are continuously calculated from the measured absorption spectra as the sample circulates under varied laser illumination conditions, designated in the figure by the \emph{Exposure Condition} number corresponding to Table~\ref{Tab:OG:ExpCond}.
The sample is initially in a pure $P_{R}$ configuration, with total Cph8 concentration of 1.62 $\mu$M.
Between 28-43 minutes in the figure the sample is in a mixed initial state $\binom{R_{M0}}{F_{M0}}$ with a non-zero $P_{FR}$ population.
Over the course of the measurement series the sample is exposed to the laser sources to initiate the photoswitching reaction by either a linear, single-pulse excitation or a non-linear, dual-pulse excitation-depletion pair.
The periods under excitation-only exposure are highlighted in yellow, while the periods exposed to the excitation-depletion pair are highlighted blue.

In the figure we mark the concentrations of two spectrally distinct sub-populations of the \pr state, $R_{670}$ and $R_{655}$, named by the peak of their absorption spectra.
In all measurements the Cph8 sample is observed to be initially free of the $R_{655}$ sup-population, which gradually develops after extended periods circulating in the experimental apparatus.
The conversion of the sample is observed under complete dark circulation with only intermittent observation by the probe to minimize exposure to light, indicating that the effect is not due to photo-damage of the protein.
A similar blue-shifted ground state sub-population is observed by Larsen et.al. \cite{Kim20140417}, as discussed in Section~\ref{Sec:OG:BGPCBDyn}.
The $R_{655}$ sub-population participates in the photoswitching with the same yield as the initial $R_{670}$ population. Typically, attempts are made to complete the measurement series before significant populations of $R_{655}$ develop.


\begin{figure}
  \centering
  \includegraphics[width=5.5in]{ch-OG/Figs/Data/Fig_R1}
  \caption[Data from representative measurement series]{Charting of the measured concentration of the $P_{R}$ and $P_{FR}$ states of Cph8 protein over the course of several measurement series under varied exposure conditions, labeled by number corresponding to Table~\ref{Tab:OG:ExpCond}. Regions highlighted yellow are exposed to the excitation pulse alone, regions highlighted blue are exposed to the excitation-depletion pulse combination, and non-highlighted regions have no laser exposure.Two spectrally distinct sub-populations of \pr are charted in the figure, $R_{655}$ and $R_{670}$, discussed in the text.}\label{R1}
\end{figure}
%Data 20160715

The first feature of note in the figure is the steady decrease of the total concentration of Cph8 protein in the sample (orange trace in Figure~\ref{R1}). Over the course of the measurement series the total protein concentration falls 14\%.
This decline in total protein concentration is seen under all conditions of circulation, including complete darkness, and is unrelated to the laser exposure.
The source and nature of the sample degradation are not investigated in this work, though there are two suspected causes.
The first is aggregation of the protein complexes, which then fall out of solution and are trapped in the sample reservoir, reducing the overall concentration.
The second is denaturation of the protein due to age, handling, or environmental conditions.
The development of the $R_{655}$ sub-species does not appear to be associated with the protein loss, as the two effects develop with a different time dependence and are believed to be unrelated processes.
Regardless of the source of the non-optical protein loss, the trend is linear and consistent across measurement series, and can be fit and removed from the measurements without adversely affecting the data.
The removal of this gradual non-optical loss trend is the first step in the processing of a measurement series.
%\tcg{Over the course of the measurement series the sample periodically circulates with no laser exposure to return to a pure $P_{R}$ initial state and measure the total Cph8 protein concentration. These points are fit to calculate the time dependent measure of the total Cph8 protein concentration in the sample over the course of the measurement series, and all measured $P_{R}$ and $P_{FR}$ concentrations are converted to ratios of this time dependent total Cph8 concentration to give the relative state populations.  This procedure is used instead of referencing the measured total Cph8 shown in Figure~\ref{R1} by the orange trace because this measurement is the post-exposure Cph8 concentration (the sum of the measured \pr and \pfr product concentrations), which includes sample loss due to photo-damage during the exposure. The dips associated with photo-damage are just visible in Figure~\ref{R1} in the regions under laser exposure.}\tcr{ $<$ Too much unnecessary detail? }

Next, the populations of the $P_{R}$ and $P_{FR}$ states are averaged over a fixed time period under each exposure condition after the measured concentration levels have stabilized. When there is a change in exposure condition it takes time for the newly exposed sample to flow through the SFC and fill the absorption cell. The final product concentrations associated with that exposure condition can not be measured until the new sample fully replaces the old. When the system stabilizes and the concentrations of the $P_{R}$ and $P_{FR}$ states are measured for one exposure condition, the condition can be switched to another in the series and a new measurement commences. Once a \emph{Full Data Set} has been measured under a given set of experimental control parameters, the \emph{characteristic coefficients} of that parameter set can be calculated and the experimental control parameters can be varied to the next point in the survey.
In practice, the collection of a \emph{Full Data Set} for a given laser parameter setting need not be measured consecutively or in any particular order, so long as all six exposure conditions are measured under similar experimental conditions to reliably calculate all six characteristic coefficients and fully describe the photoswitching reaction at that laser parameter setting and predict the final equilibrium population. In the present experiments the order of data collection was alternated to suppress systematic errors.

\begin{figure}
  \centering
  \includegraphics[width=5.5in]{ch-OG/Figs/Data/Fig_R2}
  \caption[Processed Data from representative measurement series]{Processed measurement series: The relative decrease of \pr, $(1-R/C_{Tot})$, overlaps with the relative increase of \pfr, ($F/C_{Tot}$), where $C_{Tot}$ is the total Cph8 concentration, demonstrating `clean' switching between the two states with little loss to photo-damage. As in Figure~\ref{R1}, \emph{Exposure Conditions} are labeled corresponding to Table~\ref{Tab:OG:ExpCond}: yellow regions are exposed to the excitation pulse, blue regions are exposed to the excitation-depletion pulse combination, and non-highlighted regions have no laser exposure. The bracketed region from 27-60 minutes defines one \emph{Full Data Series} collected at $\langle P_{Ex}\rangle\!\!=\!\!600\mu W$, $\langle P_{Dep}\rangle\!\!=\!\!4.5mW$, and $\uptau_{Ex,Dp}\!\!=\!\!0.5ps$ (full control parameters listed in the text).}\label{R2}
\end{figure}

Processed data from the same measurement series shown in Figure~\ref{R1} are presented in Figure~\ref{R2}, where the non-optical loss trend has been fit and removed and the $P_{R}$ and $P_{FR}$ state populations plotted as ratios of the total Cph8 concentration.
The markers indicate the average state population at each specific exposure condition indexed by the experiment time at which the exposed sample travelled from the exposure cell to the absorption cell and the measured state population had stabilized.
The standard deviation of the measured concentration over the averaged interval in each exposure condition is measured and used to calculate the error of each \emph{characteristic coefficient} by propagation of uncertainty. The errors in the measured population are smaller than the marker boxes, but grow as they are propagated through the multiple calculations necessary to determine the characteristic coefficients, the OTM, and the projected photoequilibrium population.
In the processed measurement series, the overlap of the \pfr population increase with the \pr population decrease clearly illustrates the low damage coefficients.
The larger net production of $P_{FR}$ per laser exposure at the same power when starting from zero initial concentration (Exposure Condition 2, EC2), compared to when the initial concentration of $P_{FR}$ is higher (EC5) illustrates that in EC5 the forward and reverse photo-reactions are taking place simultaneously and the sample is near photoequilibrium.
The regions in Figure~\ref{R2} when the sample was exposed to the excitation-depletion pulse combination are highlighted blue (EC3 \& EC6).
Because the number of laser pulse iterations during the exposure is kept low to more rapidly scan a larger domain of laser control parameters, the Excitation+Depletion pulse combination causes the \pfr population to \emph{decrease}, rather than increase.
Referring back to Figure~\ref{Fig:MultiExp} in Section~\ref{Sec:OG:REMMulti}, this is the expected result of the SDQ mechanism when the number of laser pulse iterations per exposure is less than the number required to surpass the linear excitation.
This occurs because the SDQ mechanism functions by slowing down both the forward and reverse reactions, but slowing the reverse reaction more, enabling a greater final photoequilibrium while requiring more laser pulse iterations to reach it.
Because of the information we extract from the iterative mapping using the Optical Transformation Matrix we are able to calculate the photoequilibrium of the laser exposure without waiting for this extended period.

%This is evidence that we are achieving Stimulated Depletion Quenching of the photoswitching reactions, but not exposing the sample to sufficient laser pulses to allow the enhancement from the quenching of the reverse photoswitching reaction to overcome the decreased overall reaction rate.

The bracketed region between 27-60 minutes encloses a single \emph{Full Data Series }of measurements taken at the following experimental control parameter settings: [$\langle P_{Ex} \rangle, \langle P_{Dep} \rangle,(\lambda_0^{Ex},\Delta\lambda_{Ex} ), (\lambda_0^Dp,\Delta\lambda_{Dp} ), \uptau_{Ex,Dp}$] = [600 $\mu$W, 4.5 mW, (625 nm, 40 nm), (835 nm, 10 nm), 0.50 ps].
The two partial data series at earlier times are taken at different excitation and depletion powers.
The first partial data series is taken at $\langle P_{Ex}\rangle=400\mu W$, $\langle P_{Dep}\rangle=1.5mW$, and $\uptau_{Ex,Dp}=0.33 ps$, and the second partial data series at $\langle P_{Ex}\rangle=600\mu W$, $\langle P_{Dep}\rangle=1.5mW$, and $\uptau_{Ex,Dp}=0.5 ps$.
Though these measurements can not be used to calculate the full set of \emph{characteristic coefficients}, they are useful for showing trends in the power and delay dependence of the forward Yield and forward Quenching coefficients.
From the \emph{Full Data Series} we can calculate the full set of \emph{characteristic coefficients}:
[$Y_{R,FR}, Q_R, D_R$]=[$0.1160\pm0.0035, 0.29\pm0.02, 0.0013\pm0.0006$], and
[$Y_{FR,R}, Q_F, D_F$]=[$0.1010\pm0.003, 0.493\pm0.055, 0.0009\pm0.0009$].
The errors in the calculated \emph{characteristic coefficients} derive from propagation of the standard deviation of the measured sample concentrations through the equations for each coefficient (see Table~\ref{Tab:CharCoeff}).

We see that the forward and reverse reaction Yield coefficients, $Y_{R,FR}$ and $Y_{FR,R}$, have similar magnitude with an advantage to the forward reaction, as expected at this excitation wavelength.
The damage coefficients are very low, which was common throughout the experiments.
As stated earlier, efforts were taken to limit photo-damage and significant levels of damage (i.e., defined as a damage coefficient higher than $\sim 1.5\%$) were only seen in samples compromised by age or environment (stored for several weeks at 4$^\circ$C or overnight at room temperature).
In extended measurement series lasting $>$10 hours the photo-damage parameter would increase over the course of the experiment, but typically remained under a few percent.
The Quenching coefficient of the reverse reaction, $Q_{FR}$, is 1.7 times greater than the forward Quenching coefficient, $Q_R$, a significant enhancement factor.
%We predict that this disruption of the reverse reaction should allow increased production of the $P_{FR}$ state over time, but while surveying the parameter space we do not expose the sample long enough to allow the enhanced equilibrium to overcome the slower reaction rate.
Using the calculated characteristic coefficients, we construct the Optical Transformation Matrix and calculate the equilibrium product population from its eigensolutions.
Analytically calculating the errors of the eigensolutions of a matrix from the errors of its components is prohibitively complicated, so the eigensolution errors were numerically computed by statistics. We calculated the eigensolutions of 1000 matrixes with components defined by the measured characteristic coefficients with gaussian variations of magnitude given by the associated coefficient errors. The standard deviation of these eigensolutions gives the error on the photoequilibrium.
The projected photoequilibrium threshold of the linear excitation is $[P_{FR}]_{EQ}^{lin} = 0.54\pm0.09$. Based on the Quenching coefficients calculated from the measurements of the full data series in Figure~\ref{R2} the projected SDQ-enhanced equilibrium threshold is $[P_{FR}]_{EQ}^{SDQ} = 0.62\pm 0.10$. This is an increase of the maximum \pfr population by 13\% or a decrease of the minimum  residual \pr population by 21\%, a sizeable enhancement.
%\tcr{Not the most dramatic example to start with, Other measurements have better threshold, but less "photogenic" for figs above (Full Data Set scattered across many measures).}

In the following section we present the calculated \emph{characteristic coefficients} measured over a range of laser parameter settings and discuss the functional dependence of the photoswitching reaction on the experimental control parameters.


%\tcr{============================}
%
%\tcr{\emph{Everything below is more like "Discussion: Experimental Difficulties" Doesn't really belong in Data Collection/processing.} }
%
%Attempts were made to increase the number of laser pulses accumulated during the exposure of the switches, but we were unable to increase the pulse count enough to see the final $P_{FR}$ product concentration under Quenching enhanced exposure rise above the $P_{FR}$ produced by linear, single beam exposure. The laser repetition rate is fixed at 1 KHz, therefore the only way to increase the number of pulses per exposure is to decrease the flow rate through the sample circuit.
%Lowering the driving voltage of the piezoelectric pump slowed the flow, but below a critical driving pressure the circuit flow would become irregular and erratic. Adding lengths of narrow diameter tubing to the circuit to provide increased resistance at higher driving voltages led to erratic flow conditions and clogs that halted circulation.
%
%The photo-isomerization reaction is very sensitive to the accumulated dose of laser excitation, and while much effort was put into maintaining consistent laser pulse energy and beam overlap, we did not have the same level of control over the sample makeup or the flow rate. This lack of control meant that exposure conditions were not consistently reproducible.Although decreases in protein concentration due to the non-optical sample degradation could be fit, removing the effects of the time-varying total protein concentration during processing of th absorption spectra, the sample degradation still had detrimental effects on the measurements. First, when comparing the transmitted beam at the start and end of a measurement series a distinctly greater amount of scatter was seen. This scatter from the degraded protein remaining in the sample solution reduced the effective power of the exposure to the photo-active Cph8 protein. Second, the altered sample makeup appeared to change the viscosity of the sample solution, altering the flow properties of the fluid circuit. The microchannel exposure cell is very sensitive to solution viscosity. When measuring the flow rate through the system to calibrate piezo micro-pump driving voltage there was a measureable difference in flow rate when circulating samples of distilled water, TKKG buffered saline solution, and actual protein sample (80\% TKKG buffer and 20\% protein concentrate in buffer solution). Slight variations in solution makeup could affect the viscosity and flow rate, affecting the number of laser pulses during the exposure.
%
%In practice, over the course of several hours the sample flow rate and other exposure conditions were typically stable enough to measure multiple full data series by which we could compare trends and conserved relationships between \emph{Characteristic Coefficients} of the photoswitching reactions measured under a series of experimental control parameters. However, variations in the uncontrolled experimental conditions reduced the precision of measurements, limiting the ability to make quantitative comparisons of measurements taken on different sample preparations over different days. Future attempts to improve the apparatus must include a means of continuously measuring the sample flow rate, both to calculate accumulated dose and to spot changes in the sample characteristics.

%\emph{\textcolor[rgb]{0.00,0.00,1.00}{MOVE VVV THIS TO END??}}
%
%The experimental results presented in Section~\ref{Sec:OG:Results} agree well with most aspects of the rate equation model: particularly the dependence of the SDQ enhancement on the power and wavelength of the excitation and depletion laser pulses, and iterative dependence on the number of laser pulse exposures.
%The experimentally measured pulse delay dependence is not in good agreement with the REM model, observing greater SDQ enhancement of the photoequilibrium state at longer excitation-depletion pulse delays where the REM simulations predict the enhancement will have diminished. The discrepancy between the model and the measured response is not unexpected, as the model does not incorporate the coherent dynamics of the molecule.
%%%  MOVE ^^^ THIS TO END
%%%

